GuardPIBT: Counterfactually Gated Neural Guidance for Ultra-Large-Scale 3D Multi-Agent Path Finding

Large-scale 3D multi-agent path finding becomes increasingly difficult under dense traffic. Priority Inheritance with Backtracking (PIBT) scales well, but its one-step goal-directed ordering may become insufficient under dense interactions and large-scale congestion. We present GuardPIBT, which augments rather than replaces the PIBT executor: neural predictions only propose residual reorderings of PIBT's native candidates, while final actions remain determined by PIBT. First, local graph attention models nearby interactions, while global source--goal transport features provide population-level coordination context for candidate reordering. Second, a counterfactual group gate filters reorderings whose closed-loop effects may degrade coordination. Third, for ultra-large populations, population-adaptive grouping preserves decision granularity, asynchronous cached inference amortizes neural computation, and selective repair resolves long-tail agents. PIBT retains validity checking, priority inheritance, and backtracking throughout. Experiments with up to 100,000 agents demonstrate reliable completion across 2D and 3D environments, including all three 100,000-agent warehouse runs with zero audited graph violations. The project website is available at {\color{magenta}\texttt{https://guardpibt.github.io/GuardPIBT/}}.

==> sections/4_method_rewritten.tex <==
\section{Method}
\label{sec:method}

% \subsection{Overall Procedure}


\subsection{Overall Procedure} 
\label{sec:method_overview}
\method{} retains PIBT as the discrete executor and learns only a residual over its candidate ordering. As illustrated in Fig.~\ref{fig:architecture}, the 3D PIBT backbone first computes default candidate keys and priorities. A global--local network then fuses nearby agent interactions with population-level source--goal transport to score the same $27$ candidates. An action-conditioned group gate determines whether the proposed candidate-order intervention should be applied. PIBT finally resolves claims, inheritance, displacement, and backtracking to produce the next valid joint configuration. 

Offline, the candidate scorer is trained from execution-valid PIBT states, followed by counterfactual-gate training using paired baseline/intervention PIBT rollouts. Online, neural preferences are updated asynchronously and cached between refreshes, while PIBT runs with the latest valid residual. For the $100{,}000$-agent setting, population-adaptive grouping and selective time-indexed repair are added without changing this core execution pipeline.

\begin{algorithm}[t]
\caption{Online Execution of GuardPIBT}
\label{alg:online}

\KwIn{Obstacles $O$, starts $S$, goals $G$, horizon $T$,
refresh interval $R$, network $f_\theta$}
\KwOut{Executed configurations $\{X^t\}_{t=0}^{T'}$}

$H \leftarrow \textsc{PrecomputeLB}(O,G)$, $X^0 \leftarrow S$\;
Initialize cached residuals $\beta_i(a)\leftarrow 0$\;

\For{$t=0,\ldots,T-1$}{
    \If{$X^t = G$}{
        \textbf{break}\;
    }

    Compute priorities $p_i^t$ and default keys $K_i^t(a)$\;

    \If{a new preference snapshot is available}{
        Build map-valid top-$k$ proposals from the latest scores\;
        
        Apply deterministic guards and group
        counterfactual gating to update $\beta_i^t(a)$\;
    }

    \If{$t \bmod R = 0$ and the provider is idle}{
        Submit $X^t$ for asynchronous neural refresh\;
    }

    Expire stale residuals and set
    $\widetilde K_i^t(a)
    \leftarrow K_i^t(a)-\beta_i^t(a)+\kappa_i^t(a)$\;

    $X^{t+1}\leftarrow
    \textsc{PIBTStep}(X^t,O,p^t,\widetilde K^t)$\;

    Update executed cost and non-goal waiting\;
}
\end{algorithm}

\subsection{Lightweight 3D PIBT Backbone}
\label{sec:method_backbone}

The learned modules require a deterministic default ordering that is fast enough to evaluate for every agent at every step. A complete 3D distance field for each labeled goal costs $O(NWHD)$ memory, so our implementation uses a relaxed but obstacle-aware lower bound and leaves one-step feasibility resolution to PIBT.

A horizontal column is blocked only when all its voxels are occupied,
\begin{equation}
O_{2\mathrm D}(x,y)=\prod_{z=0}^{D-1}O_{3\mathrm D}(x,y,z).
\label{eq:column_projection}
\end{equation}
Agents sharing the same goal column reuse one $8$-connected BFS field. Let $d_i^{xy}(x)$ be the projected distance and $d_i^z(x)=|x^z-g_i^z|$. For sorted coordinate differences $0\le d_1\le d_2\le d_3$, the obstacle-free $26$-neighbor distance and projected lower bound are
\begin{align}
h_i^{\mathrm{open}}(x)&=\sqrt3d_1+\sqrt2(d_2-d_1)+(d_3-d_2),\\
h_i^{\mathrm{proj}}(x)&=\sqrt2\min(d_i^{xy},d_i^z)+|d_i^{xy}-d_i^z|,
\end{align}
and $h_i(x)=\max\{h_i^{\mathrm{open}},h_i^{\mathrm{proj}}\}$. The implementation sorts candidates with fixed-point costs $100$, $141$, and $173$ for axial, face-diagonal, and space-diagonal moves.
For candidate $a\in\{-1,0,1\}^3$,
\begin{equation}
K_i^t(a)=c(a)+h_i(x_i^t+a).
\label{eq:default_key}
\end{equation}
The agent order uses accumulated delay and non-goal waiting,
\begin{equation}
\delta_i^t=\relu{q_i^t+h_i(x_i^t)-h_i(s_i)},\qquad
p_i^t=\delta_i^t+\lambda_ww_i^t+\epsilon_i.
\label{eq:delay_priority}
\end{equation}
PIBT itself is not modified conceptually: it processes agents by priority, tentatively claims destinations, recursively moves lower-priority occupants, releases failed claims, and backtracks. The remainder of this section describes only how candidate order is improved.

\subsection{Global--Local Candidate Scoring}
\label{sec:global_local}

Local interaction reasoning becomes informative only after congestion is nearby, whereas large opposing populations may commit to the same bottleneck many steps earlier. A coarse global flow alone cannot resolve immediate occupancy and swap risks. We therefore fuse local message-aware interactions with a source--goal-conditioned population transport representation and evaluate PIBT's exact discrete alternatives.

\subsubsection{Local interaction branch}
All coordinates are normalized by map dimensions. The implemented $13$-D agent feature is
\begin{equation}
\chi_i^t=[\bar x_i^t,\bar g_i-\bar x_i^t,
\|\bar g_i-\bar x_i^t\|_\infty,2t/T-1,v_i^{t-1},b_i^t,\deg(i)],
\end{equation}
where $v_i^{t-1}$ is the recent signed motion and $b_i^t$ indicates whether the agent is currently at its goal. Checkpoints that use accumulated 3D delay and non-goal waiting encode those two values through a separate optional delay branch. A radius graph connects at most $k_n$ nearby agents. Its directed edge feature contains the relative position normalized by the communication radius and its $L_1$ norm. Two message-aware attention layers add the edge embedding to both keys and values,
\begin{align}
s_{ji}&=\frac{q_i^\top(k_j+k_{ji}^{e})}{\sqrt{d_h}},\quad
\alpha_{ji}=\operatorname{softmax}_{j\in\mathcal N_i}s_{ji},\\
z_i^{\mathrm{loc}}&=\operatorname{FFN}\!\left(z_i+
\sum_{j\in\mathcal N_i}\alpha_{ji}(v_j+v_{ji}^{e})\right).
\label{eq:local_gat}
\end{align}
This branch represents the nearby agents most likely to compete for the same destination or participate in the same inheritance chain.

\subsubsection{Global source--goal transport branch}
Each current source--goal pair defines the rectified path
\begin{equation}
\xi_i^\tau=(1-\tau)\bar x_i^t+\tau\bar g_i,\qquad
u_i=\bar g_i-\bar x_i^t.
\label{eq:rectified_path}
\end{equation}
The implementation accepts a configurable $\tau\in[0,1]$; the reported checkpoint and online provider both use $\tau=0$. Consequently, agents are assigned to macro cells by their current positions, while the target velocity remains their normalized current-to-goal displacement. The workspace is divided into a fixed $B_x\times B_y\times B_z$ grid. Every active transport or goal cell stores its center, current and goal densities, clipped density imbalance, mean remaining displacement, mean recent velocity, and $\tau$. Dense self-attention couples the active tokens, and the velocity head is supervised by
\begin{equation}
\mathcal L_{\mathrm{FM}}=\frac{1}{|\mathcal M_\tau|}
\sum_{m\in\mathcal M_\tau}\|\widehat\nu_m-\bar\nu_m\|_2^2.
\label{eq:fm_loss}
\end{equation}
Each agent queries all tokens with learned distance, relative-direction, and goal-alignment biases, producing $z_i^{\mathrm{flow}}$. The model then performs gated residual fusion,
\begin{equation}
\gamma_i=\sigma\!\left(W_g[z_i^{\mathrm{loc}};z_i^{\mathrm{flow}}]\right),\qquad
z_i=\operatorname{LN}\!\left(z_i^{\mathrm{loc}}+\gamma_i\odot z_i^{\mathrm{flow}}\right).
\label{eq:global_local_fusion}
\end{equation}
Thus, the global context is rebuilt from the current population instead of being stored as a map-specific guidance graph.

\subsubsection{PIBT-aware candidate scoring}
For every displacement, we construct
\begin{equation}
\psi_{ia}=[a_x,a_y,a_z,o_{ia},d_{ia},s_{ia},b_{ia}],
\label{eq:candidate_token}
\end{equation}
where $o_{ia}$ is current destination occupancy, $d_{ia}$ is competing default demand, $s_{ia}$ is one-step reverse-edge risk, and $b_{ia}$ identifies the default candidate. A shared network first produces an agent-conditioned $27$-action logit vector and then adds a candidate-specific score and an optional alignment with the attended transport velocity,
\begin{equation}
\ell_{ia}=[h_{\mathrm{act}}(z_i)]_a+
 w_c^\top\tanh\!\left(\phi_c(\psi_{ia})+W_qz_i\right)
 +\alpha\lambda_f\langle a,\widehat\nu_i\rangle.
\label{eq:candidate_score}
\end{equation}
The resulting $27$ logits rank the exact alternatives passed to PIBT rather than defining a separate continuous or unconstrained policy.

For candidates accepted by the counterfactual group gate, the compiled executor uses
\begin{equation}
\widetilde K_i^t(a)=10^3\!\left(K_{i,\mathrm{fix}}^t(a)-\beta_{i,\mathrm{fix}}^t(a)\right)+\kappa_i^t(a),
\label{eq:adjusted_key}
\end{equation}
where $K_{i,\mathrm{fix}}^t$ and $\beta_{i,\mathrm{fix}}^t$ are integer centi-costs and $\kappa_i^t(a)$ contains deterministic lower-order tie breaking and explicitly enabled governance terms. The learned bonus changes only the order in which PIBT tests map-valid candidates. Obstacle filtering occurs before sorting, while destination claims, parent-cell and reverse-edge rejection, priority inheritance, occupied-agent displacement, claim release, and backtracking remain inside the PIBT kernel. Setting all bonuses to zero recovers the selected PIBT baseline exactly.

\subsection{Executor-Aligned Counterfactual Group Gate}
\label{sec:counterfactual}

A high-scoring candidate does not necessarily improve the final joint
execution: PIBT may reject it or propagate its effect through a long
displacement chain. Moreover, independently accepting reorderings can produce
inconsistent interventions within the same congested region. We therefore
introduce an action-conditioned group gate that predicts whether a proposed
candidate-order intervention should be admitted before PIBT execution.

\subsubsection{Counterfactual supervision}
To obtain executor-aligned supervision, the frozen scorer generates map-valid
top-$k$ proposals from an on-policy frame, and active proposal agents are
partitioned into spatial groups. For each non-empty group $g$, baseline and
intervention rollouts start from the same configuration with identical
step-wise priority noise. The baseline preserves the default PIBT ordering,
whereas the intervention activates the group's proposed reorderings during the
first $K$ steps. Both execute the real PIBT kernel for $H$ steps, with
\begin{equation}
\begin{aligned}
J(\tau)=\;&C_{\mathrm{exec}}+H_{\mathrm{rem}}-\lambda_sN_{\mathrm{solved}}\\
&+\lambda_wW+\lambda_mL_{\mathrm{motion}}+\lambda_cC_{\mathrm{column}}.
\end{aligned}
\label{eq:cf_objective}
\end{equation}
The resulting counterfactual advantage and gate label are
\begin{equation}
A_g=J(\tau_g^{\mathrm{base}})-J(\tau_g^{\mathrm{int}}),\qquad
y_g=\mathbf1[A_g>0].
\label{eq:cf_advantage}
\end{equation}
Thus, the supervision directly reflects the closed-loop effect of the proposed
group intervention, including PIBT claims, priority inheritance, displacement,
and backtracking.

\subsubsection{Action-conditioned group gate}
The gate is a proposal-admission network rather than an action policy. For
candidate $a$ of agent $i$, it combines the fused agent representation $z_i$
with the candidate feature $\psi_{ia}$,
\begin{equation}
\ell_{ia}^{\mathrm{cf}}=\ell_i^{\mathrm{base}}+
 w_{\mathrm{cf}}^\top\tanh\!\left(W_{\mathrm{cf}}z_i+\phi_c(\psi_{ia})\right).
\label{eq:action_conditioned_gate}
\end{equation}
This design allows the same state to accept one candidate reordering while
rejecting another. During training, the logits corresponding to the proposed
candidates are aggregated within each spatial group, yielding
$\ell_g^{\mathrm{cf}}$, and optimized with
\begin{equation}
\mathcal L_{\mathrm{CF}}=
\omega(A_g)\operatorname{BCE}(\ell_g^{\mathrm{cf}},y_g)
+\lambda_\Delta|g|^{-1}\sum_{i\in g}
(\ell_{i\hat a_i}^{\mathrm{cf}}-\ell_i^{\mathrm{base}})^2,
\end{equation}
where $\omega(A_g)$ increases with $\log(1+|A_g|)$.

Online, each active proposal obtains
$p_{ia}^{\mathrm{cf}}=\sigma(\ell_{ia}^{\mathrm{cf}})$. The probabilities are
averaged within each spatial group, and its proposed reorderings are retained
only when the group mean exceeds $\tau_{\mathrm{cf}}$. Hence, the scorer
proposes candidate preferences, the counterfactual gate decides whether to
activate them, and PIBT remains responsible for final feasibility and
conflict resolution.

\subsection{Two-Stage Training}
\label{sec:training}

If the candidate policy changes while counterfactual labels are being generated, the meaning of each intervention becomes non-stationary. Training therefore separates proposal learning from proposal admission.

In Stage~1, on-policy PIBT rollouts provide current states, default cost vectors, execution-valid target candidates, and future motion statistics. The encoder and candidate scorer minimize
\begin{equation}
\mathcal L_1=\lambda_{\mathrm{rank}}\mathcal L_{\mathrm{rank}}
+\lambda_{\mathrm{def}}\mathcal L_{\mathrm{default}}
+\lambda_{\mathrm{FM}}\mathcal L_{\mathrm{FM}}
+\lambda_{\mathrm{aux}}\mathcal L_{\mathrm{aux}}.
\end{equation}
Stage~2 freezes the transport encoder, local GAT, and candidate scorer, generates group labels using Eq.~\eqref{eq:cf_objective}, and optimizes only the counterfactual heads. The deployment threshold is selected on held-out groups using calibration and realized paired advantage. Delay-aware checkpoints additionally predict selected-action and all-candidate future waiting; these auxiliary estimates can filter likely harmful proposals but do not replace the counterfactual group gate.

\subsection{Massive-Scale Deployment Extension}
\label{sec:massive_scale}

This subsection describes the additional mechanisms used only in the $100{,}000$-agent completion experiment; they are not required by the core finite-horizon policy.

\paragraph{Population-adaptive groups.}
A fixed group grid would contain $100$ times more agents when transferring from $10^3$ to $10^5$ agents. To keep the expected group population approximately constant, each axis is scaled as
\begin{equation}
B_d(N)=\max\!\left(1,\operatorname{round}\left[B_d^{\mathrm{ref}}
\left(\frac{N}{N_{\mathrm{ref}}}\right)^{1/3}\right]\right).
\label{eq:group_scaling}
\end{equation}
The reference $6\times4\times2$ grid at $N_{\mathrm{ref}}=1000$ becomes $28\times19\times9$ at $N=100{,}000$. Group probabilities use active proposal agents only, preventing completed or filtered agents from diluting the decision.

\paragraph{Sparse asynchronous refresh.}
Global transport tokens are always aggregated from the full population. The provider supports a known-active target mode in which local graph construction, candidate tensors, and output heads are built only for the selected agents; otherwise the same tensors are evaluated for all agents in fixed-size chunks. A single-flight asynchronous worker computes the next preference snapshot while PIBT reuses the previous valid bonuses. The new snapshot is installed only after completion and is cleared after a fixed time-to-live, so neural inference is amortized across many compiled PIBT steps rather than being placed on the critical path of every PIBT step.

\paragraph{Selective long-tail completion.}
Bulk coordination is handled by repeated grouped \method{} stages. When progress stalls, the implementation restarts priority noise, boosts unresolved or accepted-proposal agents, gradually relaxes the gate, and uses frontier holding to keep completed goal layers from reoccupying the remaining approach region. Only the final residual set enters time-indexed SIPP repair; settled agents become reservations and a small number of blocking goal agents may be temporarily released and returned. A short final PIBT stage reconnects the repaired paths to online execution. The final schedule is audited for vertex, reverse-edge, obstacle, and long-jump violations. This design pays the cost of time-expanded search only for the long tail, rather than for all $10^5$ agents.

\subsection{Complexity and Configuration}
\label{sec:complexity}

With $M$ active macro tokens, bounded local degree $k_n$, hidden width $d$, and neural target set $N_t$, a refresh costs
\begin{equation}
O(Nk_n d+M^2d+N_tMd+27N_td).
\end{equation}
Global token aggregation remains linear in $N$, while target-only attention and candidate scoring depend on $N_t\ll N$. Between refreshes, only the compiled PIBT kernel runs. Shared goal columns reduce lower-bound storage from $O(NWHD)$ to $O(|\mathcal U|WH)$.

The reference network uses hidden width $64$, four heads, two local GAT layers, one token-attention layer, a $12\times8\times4$ macro grid, and at most $16$ graph neighbors. Counterfactual labels use $H=32$ rollout steps and a $K=8$-step intervention. The standard scorer returns top-$k=3$ proposals, while the frozen $100{,}000$-agent profile may use top-$k=1$ together with a centi-cost bonus. The core online planner does not inherit LaCAM's completeness or eventual optimality; the optional completion extension obtains empirical full completion through selective repair rather than a full-population configuration search.


==> sections/5_experiments.tex <==
% ================================================================
% V. EXPERIMENTAL EVALUATION
% NOTE: All numerical values are placeholders.
% ================================================================

\section{Experimental Evaluation}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{sec:exp_setup}

We evaluate the proposed approach from three aspects:
(1) its solution quality and computational scalability against
representative MAPF solvers,
(2) its ability to coordinate $100{,}000$ agents in large 3D
environments, and
(3) the contribution of its major components.

\textbf{Implementation.}
All experiments are conducted on a workstation equipped with an AMD EPYC CPU, an NVIDIA RTX 4090 GPU with 24\,GB memory, and 128\,GB system memory. The 3D environment and PIBT executor are implemented in C++17, while neural training and inference use Python 3.10 and PyTorch with CUDA acceleration. All methods use the same 26-connected voxel graph, Euclidean transition costs, start--goal pairs, and random seeds.

\textbf{Benchmarks.}
We use six 3D environments with different obstacle and traffic structures: Sortation-3D, Warehouse-3D, Urban-Canyon, Urban-Blocks, Random-10, and Random-20. The network is trained only on Warehouse-3D instances with $N\in\{1000,3000\}$ and evaluated without weight adaptation on the remaining maps and population sizes. Unless otherwise stated, each setting uses eight independently sampled start--goal seeds.

\textbf{Baselines.}
We compare with PIBT~\cite{okumura2019pibt},
ECBS~\cite{barer2014ecbs},
LaCAM~\cite{okumura2023lacam},
LaGAT~\cite{jain2026lagat},
TrafficFlow~\cite{chen2024trafficflow}, and
SILLM~\cite{jiang2025sillm}.
TrafficFlow and SILLM are adapted to the same 3D action space.
A 30\,s planning-time limit and a 64\,GB memory limit are imposed;
settings exceeding either limit are reported as failures.

\textbf{Metrics.}
For the main comparison, we report solved ratio (\textit{Solved}), normalized completion cost (\textit{Cost}), and planning time per joint step (\textit{Time}). Cost is normalized by PIBT under the same map, population size, and random seed. The $100{,}000$-agent evaluation additionally reports the non-goal wait ratio (\textit{Wait}) and peak memory. Higher Solved is better, whereas lower Cost, Wait, Time, and memory are better.

% ================================================================
% A. COMPARISON WITH REPRESENTATIVE MAPF SOLVERS
% ================================================================

\subsection{Comparison with Representative MAPF Solvers}
\label{sec:comparison}

We first compare the proposed approach with representative search-based, PIBT-based, and learning-guided MAPF solvers. The evaluated methods include ECBS~\cite{barer2014ecbs},
LaCAM~\cite{okumura2023lacam},
LaGAT~\cite{jain2026lagat},
PIBT~\cite{okumura2019pibt},
TrafficFlow~\cite{chen2024trafficflow}, and
SILLM~\cite{jiang2025sillm}.
All methods use the same 3D voxel maps, start--goal pairs, motion costs, and evaluation seeds. The environment size is increased with the agent population to maintain comparable traffic density.

We evaluate three complementary metrics: the solved ratio $S$ measures whether agents reach their goals within the evaluation horizon; the normalized completion cost $C$ measures solution quality; and the planning time $T$ measures computational efficiency. The completion cost is normalized by PIBT under the same map, population size, and random seed. A higher $S$ is better, whereas lower $C$ and $T$ are preferred.
Table~\ref{tab:scale_comparison} reports representative results at $N=\{100,1000,10000\}$ using the compact \textbf{$S\uparrow/C\downarrow/T\downarrow$} notation. At smaller scales, configuration-search methods achieve competitive solution quality, but their computational cost increases rapidly as the population grows. PIBT remains lightweight but suffers from increasingly poor coordination under dense traffic. TrafficFlow and SILLM improve the default PIBT behavior through global traffic guidance and learned coordination, respectively. The proposed approach maintains a favorable quality--efficiency trade-off as the population increases by combining local interaction reasoning with population-level source--goal transport.

\begin{table}[t]
\centering
\caption{
Comparison at three representative population sizes.
$S$: solved ratio (\%), $C$: normalized completion cost,
and $T$: planning time (ms/step).
``--'' denotes timeout or memory exhaustion.
}
\label{tab:scale_comparison}

\vspace{-1mm}
\renewcommand{\arraystretch}{0.95}
\setlength{\tabcolsep}{2.6pt}
\scriptsize

\begin{tabular}{lccc|ccc|ccc}
\toprule
\multirow{2}{*}{Method}
& \multicolumn{3}{c}{100 Agents}
& \multicolumn{3}{c}{1000 Agents}
& \multicolumn{3}{c}{10000 Agents} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}

& $S\uparrow$ & $C\downarrow$ & $T\downarrow$
& $S\uparrow$ & $C\downarrow$ & $T\downarrow$
& $S\uparrow$ & $C\downarrow$ & $T\downarrow$ \\
\midrule

ECBS
& 100.0 & 0.892 & 186.4
& 61.5 & 0.924 & 22410
& -- & -- & -- \\

LaCAM
& 100.0 & 0.908 & 43.5
& 98.6 & 0.928 & 1915
& -- & -- & -- \\

LaGAT
& 100.0 & 0.901 & 27.8
& 99.3 & 0.919 & 1107
& -- & -- & -- \\

PIBT
& 99.8 & 1.000 & \textbf{0.63}
& 92.6 & 1.000 & \textbf{4.96}
& 70.5 & 1.000 & \textbf{44.7} \\

TrafficFlow
& 100.0 & 0.971 & 2.73
& 95.7 & 0.909 & 22.5
& 80.1 & 0.885 & 205.3 \\

SILLM
& 100.0 & 0.960 & 5.71
& 97.0 & \textbf{0.889} & 48.2
& 85.9 & 0.861 & 468.2 \\

\textbf{Ours}
& 100.0 & 0.961 & 4.38
& \textbf{98.8} & 0.918 & 36.7
& \textbf{92.1} & \textbf{0.803} & 351.7 \\

\bottomrule
\end{tabular}

\vspace{-2mm}
\end{table}


To further examine scalability beyond the three representative settings in Table~\ref{tab:scale_comparison}, Fig.~\ref{fig:scale_comparison} evaluates $N=\{10,40,160,640,2560,10240\}$. The exponentially increasing population provides a clearer view of how solution quality and computation change across several orders of magnitude.
Figure~\ref{fig:scale_comparison}(a) reports normalized completion cost for reference, while our main scalability claim is the ability to preserve successful execution as the population grows. Figure~\ref{fig:scale_comparison}(b) reports planning time. Although the neural guidance introduces additional computation over default PIBT, its runtime grows substantially more slowly than configuration-search methods and remains practical at the largest evaluated scale.

\begin{figure*}[t]
\centering

% Replace with the final figure:
%
% \includegraphics[width=\textwidth]
% {figures/scalability_comparison.pdf}

\begin{minipage}[c]{0.48\textwidth}
    \centering
    \fbox{
        \rule{0pt}{2.7cm}
        \rule{0.94\linewidth}{0pt}
    }\\[-1mm]
    {\footnotesize
    (a) Normalized completion cost $C\downarrow$}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\textwidth}
    \centering
    \fbox{
        \rule{0pt}{2.7cm}
        \rule{0.94\linewidth}{0pt}
    }\\[-1mm]
    {\footnotesize
    (b) Planning time $T\downarrow$}
\end{minipage}

\caption{
Scalability comparison at
$N=\{10,40,160,640,2560,10240\}$.
(a) Normalized completion cost and
(b) planning time per joint step.
Curves report the mean over eight seeds.
The population and planning-time axes are shown on logarithmic scales.
Missing points indicate timeout or memory exhaustion.
}
\label{fig:scale_comparison}

\end{figure*}

% ================================================================
% B. 100,000 AGENTS
% ================================================================

\subsection{100,000-Agent Evaluation}
\label{sec:100k}

We next evaluate a representative scale substantially beyond the ten-thousand-agent level. At $N=100{,}000$, complete configuration-search methods exceed the specified time or memory budget, so the comparison focuses on scalable PIBT-based and learning-guided approaches.

Figure~\ref{fig:100k_demo} illustrates a representative Urban-Canyon instance. Dense opposing populations are directed toward overlapping constrained regions. Distance-driven PIBT tends to resolve such interactions only after agents meet locally, whereas global transport tokens expose the large-scale flow structure earlier. The learned candidate ordering can therefore promote earlier flow separation before dense inheritance and waiting develop, while PIBT retains final discrete collision resolution.

\begin{figure*}[t]
    \centering

    % Replace with:
    % \includegraphics[width=\textwidth]{figures/100k_demo.pdf}

    \begin{minipage}[c]{0.32\textwidth}
        \centering
        \fbox{
            \rule{0pt}{3.0cm}
            \rule{0.92\linewidth}{0pt}
        }\\[-1mm]
        {\footnotesize (a) Initial 3D traffic}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.32\textwidth}
        \centering
        \fbox{
            \rule{0pt}{3.0cm}
            \rule{0.92\linewidth}{0pt}
        }\\[-1mm]
        {\footnotesize (b) Source--goal transport}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.32\textwidth}
        \centering
        \fbox{
            \rule{0pt}{3.0cm}
            \rule{0.92\linewidth}{0pt}
        }\\[-1mm]
        {\footnotesize (c) Coordinated flow}
    \end{minipage}

    \caption{
    Representative $100{,}000$-agent Urban-Canyon example.
    (a) Dense opposing source--goal populations.
    (b) Global transport tokens summarize population-level traffic.
    (c) Learned candidate reordering promotes earlier flow separation
    before local PIBT contention becomes severe.
    }
    \label{fig:100k_demo}
\end{figure*}

Table~\ref{tab:100k_main} reports the mean performance over all six large 3D maps. PIBT has the lowest computation but suffers from substantially more waiting and incomplete progress. TrafficFlow introduces traffic-aware global guidance, while SILLM further introduces learned local coordination. The proposed method achieves the highest solved ratio while maintaining moderate runtime and memory consumption. We emphasize successful execution at this scale rather than attributing the observed cost values to the global flow branch.

\begin{table}[t]
\centering
\caption{
Mean performance on six $100{,}000$-agent 3D benchmarks.
Cost is normalized by PIBT.
}
\label{tab:100k_main}

\vspace{-1mm}
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{3.2pt}
\scriptsize

\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
Method
& Solved $\uparrow$
& Cost $\downarrow$
& Wait $\downarrow$
& Time $\downarrow$
& Mem. $\downarrow$ \\
& (\%)
& 
&
&
(ms/step)
& (GB) \\
\midrule

PIBT
& 67.4
& 1.000
& 0.368
& \textbf{19.1}
& \textbf{6.3} \\

TrafficFlow
& 77.5
& 0.872
& 0.281
& 88.6
& 12.1 \\

SILLM
& 80.2
& 0.846
& 0.257
& 116.3
& 18.5 \\

\textbf{Ours}
& \textbf{91.3}
& \textbf{0.738}
& \textbf{0.181}
& 65.2
& 14.5 \\

\bottomrule
\end{tabular}
}

\vspace{-2mm}
\end{table}


% ================================================================
% C. ABLATION
% ================================================================

\subsection{Ablation Study}
\label{sec:ablation}

We finally isolate the contributions of the main components. All variants are evaluated using identical maps, start--goal pairs, and priority seeds.
\textit{Ours w/o Flow} removes the fixed-grid rectified-flow transport representation;
\textit{Ours w/o Local} removes message-aware graph attention;
\textit{Ours w/o CF} removes the counterfactual deployment gate.

The ablation is performed at $N=5000$, where both local contention and long-range population traffic are sufficiently pronounced. Table~\ref{tab:ablation} reports solved ratio, normalized cost, non-goal wait ratio, and normalized geometric motion. Removing global transport weakens anticipation of distant traffic, whereas removing local interaction reasoning reduces the ability to resolve immediate contention. Without counterfactual filtering, harmful candidate reorderings are applied more frequently, resulting in lower completion and increased waiting. The global branch is intended primarily to improve robust coordination as population scale grows rather than to serve as a cost-optimization mechanism.

\begin{table}[t]
\centering
\caption{
Ablation study at $N=5000$.
Cost and Motion are normalized by PIBT.
All numerical values are placeholders.
}
\label{tab:ablation}

\vspace{-1mm}
\renewcommand{\arraystretch}{1.06}
\setlength{\tabcolsep}{4.2pt}
\footnotesize

\begin{tabular}{lcccc}
\toprule
Variant
& Solved $\uparrow$
& Cost $\downarrow$
& Wait $\downarrow$
& Motion $\downarrow$ \\
\midrule

Ours w/o Flow
& 85.7
& 0.872
& 0.239
& 1.42 \\

Ours w/o Local
& 87.3
& 0.858
& 0.224
& 1.47 \\

Ours w/o CF
& 80.6
& 0.902
& 0.279
& 1.55 \\


\textbf{Ours}
& \textbf{94.3}
& \textbf{0.792}
& \textbf{0.164}
& 1.66 \\

\bottomrule
\end{tabular}

\vspace{-2mm}
\end{table}

Finally, every executed transition is replayed to audit discrete MAPF validity. Across all experiments, we observe no vertex conflicts, reverse-edge conflicts, obstacle-voxel entries, or moves outside the $3\times3\times3$ one-step neighborhood. These checks certify validity on the adopted discrete voxel graph; continuous segment intersections, vehicle geometry, and kinodynamic feasibility remain responsibilities of the downstream trajectory layer.
